VLM-KD: Knowledge Distillation from VLM for Long-Tail Visual Recognition

For visual recognition, knowledge distillation typically involves transferring knowledge from a large, well-trained teacher model to a smaller student model. In this paper, we introduce an effective method to distill knowledge from an off-the-shelf vision-language model (VLM), demonstrating that it provides novel supervision in addition to those from a conventional vision-only teacher model. Our key technical contribution is the development of a framework that generates novel text supervision and distills free-form text into a vision encoder. We showcase the effectiveness of our approach, termed VLM-KD, across various benchmark datasets, showing that it surpasses several state-of-the-art long-tail visual classifiers. To our knowledge, this work is the first to utilize knowledge distillation with text supervision generated by an off-the-shelf VLM and apply it to vanilla randomly initialized vision encoders.

==> Figures/prompt.tex <==
\begin{figure*}[t*]
     \centering
     \includegraphics[width=\textwidth]{Figures/prompt.png}
     \caption{Prompt examples and responses. Prompt-1 aims to discover visual features from the entire image while Prompt-2 only describes the target object, as it includes the groundtruth.}
     \label{fig:prompt}
\end{figure*}

==> Tables/ablade_comb1.tex <==
\begin{table*}[b]
 \begin{minipage}{0.49\linewidth}
  \caption{Ablation study on text encoders under different settings. (Open-CLIP denoted as O-CLIP)}
  \centering
  \begin{tabular}{p{2.5cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}}
%   \begin{tabular}{llllll}
    \toprule
    Text Encoder & Many & Med & Few & Avg \\
    \midrule
    ProCo & 68.2 & 55.1 & 38.1 & 57.8 \\
    \midrule
    CLIP ViT-B/16 & \textbf{70.6} & 58.0 & 
    \textbf{42.1} & \textbf{60.7} \\
    CLIP ViT-L/14 & 70.6 & \textbf{58.1} & 40.4 & 60.5 \\
    O-CLIP ViT-G/14 & 70.5 & 57.9 & 40.6 & 60.4 \\
    \midrule
    MPNet~\cite{song2020mpnet} & 70.4 & 57.9 & 40.2 & 60.3 \\
    \midrule
    CLIP ViT-B/16-F  & 68.9 & 55.4 & 38.5 & 58.3 \\
    \bottomrule
  \end{tabular}
  \label{abl:text}
\end{minipage}   
~
\begin{minipage}{0.49\linewidth}
  \caption{Ablation study on different types of text supervisions.}
  \centering
  \label{abl:prompt}
  \begin{tabular}{p{2.5cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}}
%   \begin{tabular}{llllll}
    \toprule
    Method & Many & Med & Few & Avg \\
    \midrule
    ProCo & 68.2 & 55.1 & 38.1 & 57.8 \\
    \midrule
    Classname & 68.3 & 55.2 & 38.7 & 58.0 \\
    VL-LTR~\cite{tian2022vl} & 68.3 & 55.2 & 38.7 & 58.2 \\
    Prompt-short & \textbf{70.6} & 58.0 & \textbf{42.1} & \textbf{60.7}  \\
    Prompt-long & 70.4 & 57.8 & 39.0 & 60.1 \\
    Keyword-short & 69.8 & \textbf{58.1} & 40.4 & 60.2 \\
    Keyword-long & 69.5 & 58.1 & 40.9 & 60.1 \\
    \bottomrule
  \end{tabular}
\end{minipage} 
\end{table*}

==> Tables/ablade_comb2.tex <==
\begin{table*}[t]
 \begin{minipage}{0.49\linewidth}
  \caption{Ablation study on different VLMs.}
  \centering
  \begin{tabular}{p{2.5cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}}
%   \begin{tabular}{llllll}
    \toprule
    Method & Many & Med & Few & Avg \\
    \midrule
    ProCo & 68.2 & 55.1 & 38.1 & 57.8 \\
    \midrule
    Mistral-7b & \textbf{70.6} & \textbf{58.0} & \textbf{42.1} & \textbf{60.7}  \\
    Vicuna-13b & 70.4 & 57.9 & 40.2 & 60.3 \\
    Hermes-Yi-34B & 70.5 & 58.0 & 41.0 & 60.5 \\
    \bottomrule
  \end{tabular}
  \label{abl:vlm}
\end{minipage}   
~
\begin{minipage}{0.49\linewidth}
  \caption{Ablation study on different text adaptor.}
  \centering
  \label{abl:head}
  \begin{tabular}{p{2.5cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}}
%   \begin{tabular}{llllll}
    \toprule
    Method & Many & Med & Few & Avg \\
    \midrule
    ProCo & 68.2 & 55.1 & 38.1 & 57.8 \\
    \midrule
    Linear layer & 68.9 & 55.6 & 40.0 & 58.6 \\
    1xMLP + Linear & \textbf{70.6} & \textbf{58.0} & \textbf{42.1} & \textbf{60.7}  \\
    2xMLP + Linear & 70.3 & 58.0 & 40.1 & 60.1 \\
    \bottomrule
  \end{tabular}
\end{minipage} 
\end{table*}

==> Tables/app_gpaco.tex <==
\begin{table}[b]
  \caption{Comparisons on ImageNet-LT.}
  \label{app:table:imglt}
  \centering
  \begin{tabular}{p{3.75cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}}
%   \begin{tabular}{llllll}
    \toprule
    Method & Many & Med & Few & Avg \\
    \midrule
    $\tau$ -norm~\cite{kang2019decoupling} & 56.6 & 44.2 & 27.4 & 46.7  \\
    DisAlign~\cite{zhang2021distribution} & 61.3 & 52.2 & 31.4 & 52.9 \\
    GCL~\cite{li2022long} & 63.0 & 52.7 & 37.1 & 54.5 \\
    RIDE~\cite{wang2020long} & 66.2 & 51.7 & 34.9 & 54.9 \\
    BCL~\cite{zhu2022balanced} & - & - & - & 56.0 \\
    DOC~\cite{wang2022towards} & 65.1 & 52.8 & 34.2 & 55.0 \\
    DLSA~\cite{xu2022constructing} & 67.8 & 54.5 & 38.8 & 57.5 \\
    PaCo~\cite{cui2021parametric} & 64.4 & 55.7 & 33.7 & 56.0 \\
    NCL~\cite{li2022nested} & 67.3 & 55.4 & 39.0 & 57.7 \\
    GPaCo~\cite{cui2023generalized} & - & - & - & 58.5 \\
    ProCo~\cite{du2024probabilistic} & 68.2 & 55.1 & 38.1 & 57.8 \\
    \midrule
    %Ours (Local Only) & 0.1 & 56.0 & 0.1 & 57.1 & 0.1 & 0.1 & 0.1 & 58.5 \\
    GPaCo (our reproduce) & 65.9 & 55.0 & 40.6 & 57.2 \\
    GPaCo + Text & - & - & - & - \\
    GPaCo + KD-Image & 64.2 & 59.5 & 44.6 & 59.3 \\
    GPaCo + RISE & - & - & - & -\\
    GPaCo + Text + KD-Image & - & - & - & - \\
    \midrule
    CLIP ViT-B/16 & 82.2 & 73.9 & 52.8 & 74.4 \\
    \bottomrule
  \end{tabular}
\end{table}

==> Tables/imglt_bak.tex <==
\begin{table}
  \caption{Comparisons on ImageNet-LT and iNaturalist 2018 trained with different methods.}
  \label{table:main_table_imglt}
  \centering
  \begin{tabular}{p{3.75cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}|p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}}
%   \begin{tabular}{llllll}
    \toprule
    & \multicolumn{4}{c}{ImageNet-LT} & \multicolumn{4}{c}{iNaturalist 2018} \\
    \cmidrule(r){2-9}
    Method & Many & Med & Few & Avg & Many & Med & Few & Avg \\
    \midrule
    $\tau$ -norm~\cite{kang2019decoupling} & 56.6 & 44.2 & 27.4 & 46.7 & 65.6 & 65.3 & 65.9 & 65.6  \\
    DisAlign~\cite{zhang2021distribution} & 61.3 & 52.2 & 31.4 & 52.9 & 69.0 & 71.1 & 70.2 & 70.6 \\
    GCL~\cite{li2022long} & 63.0 & 52.7 & 37.1 & 54.5 & 67.5 & 71.3 & 71.5 & 71.0 \\
    RIDE~\cite{wang2020long} & 66.2 & 51.7 & 34.9 & 54.9 & 72.2 & 70.2 & 72.2 & 72.7 \\
    BCL~\cite{zhu2022balanced} & - & - & - & 56.0 & 66.7 & 71.0 & 70.7 & 70.4 \\
    DOC~\cite{wang2022towards} & 65.1 & 52.8 & 34.2 & 55.0 & 72.8 & 71.7 & 70.0 & 71.0 \\
    DLSA~\cite{xu2022constructing} & 67.8 & 54.5 & 38.8 & 57.5 & - & - & - & 72.8 \\
    PaCo~\cite{cui2021parametric} & 64.4 & 55.7 & 33.7 & 56.0 & 70.3 & 73.2 & 73.6 & 73.2 \\
    NCL~\cite{li2022nested} & 67.3 & 55.4 & 39.0 & 57.7 & 72.0 & 74.9 & 73.8 & 74.2 \\
    GPaCo~\cite{cui2023generalized} & - & - & - & 58.5 & 73.0 & 75.5 & 75.7 & 75.4 \\
    ProCo~\cite{du2024probabilistic} & 68.2 & 55.1 & 38.1 & 57.8 & 74.0 & 76.0 & 76.0 & 75.8 \\
    \midrule
    %Ours (Local Only) & 0.1 & 56.0 & 0.1 & 57.1 & 0.1 & 0.1 & 0.1 & 58.5 \\
    ProCo + Text & 70.6 & 58.0 & 42.1 & 60.7 & 75.3 & 76.6 & 76.6 & 76.5 \\
    ProCo + KD-Image & 70.7 & 58.3 & 41.6 & 60.8 & 74.9 & 76.2 & 76.2 & 76.1 \\
    ProCo + RISE & 70.8 & 58.4 & 41.7 & 60.9 & 75.0 & 76.4 & 76.5 & 76.3 \\
    ProCo + Text + KD-Image & \textbf{71.0} & \textbf{60.1} & \textbf{43.2} & \textbf{62.0} & \textbf{75.8} & \textbf{77.3} & \textbf{77.2} & \textbf{77.1} \\
    \midrule
    CLIP ViT-B/16 & 82.2 & 73.9 & 52.8 & 74.4 & 78.0 & 75.1 & 71.6 & 74.0 \\
    \bottomrule
  \end{tabular}
\end{table}

==> Tables/imglt_combine_bak.tex <==
\begin{table}[b]
  \caption{Comparisons on ImageNet-LT and iNaturalist 2018 trained with ResNet-50.}
  \label{table:main_table_imglt}
  \centering
  \begin{tabular}{p{4.00cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}|p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}}
%   \begin{tabular}{llllll}
    \toprule
    & \multicolumn{4}{c}{ImageNet-LT (ProCo)} & \multicolumn{4}{c}{iNaturalist 2018 (GPaCo)} \\
    \cmidrule(r){2-9}
    Method & Many & Med & Few & Avg & Many & Med & Few & Avg \\
    \midrule
    $\tau$ -norm~\cite{kang2019decoupling} & 56.6 & 44.2 & 27.4 & 46.7 & 65.6 & 65.3 & 65.9 & 65.6  \\
    DisAlign~\cite{zhang2021distribution} & 61.3 & 52.2 & 31.4 & 52.9 & 69.0 & 71.1 & 70.2 & 70.6 \\
    GCL~\cite{li2022long} & 63.0 & 52.7 & 37.1 & 54.5 & 67.5 & 71.3 & 71.5 & 71.0 \\
    RIDE~\cite{wang2020long} & 66.2 & 51.7 & 34.9 & 54.9 & 72.2 & 70.2 & 72.2 & 72.7 \\
    BCL~\cite{zhu2022balanced} & - & - & - & 56.0 & 66.7 & 71.0 & 70.7 & 70.4 \\
    DOC~\cite{wang2022towards} & 65.1 & 52.8 & 34.2 & 55.0 & 72.8 & 71.7 & 70.0 & 71.0 \\
    DLSA~\cite{xu2022constructing} & 67.8 & 54.5 & 38.8 & 57.5 & - & - & - & 72.8 \\
    PaCo~\cite{cui2021parametric} & 64.4 & 55.7 & 33.7 & 56.0 & 70.3 & 73.2 & 73.6 & 73.2 \\
    NCL~\cite{li2022nested} & 67.3 & 55.4 & 39.0 & 57.7 & 72.0 & 74.9 & 73.8 & 74.2 \\
    GPaCo~\cite{cui2023generalized} & - & - & - & 58.5 & 73.0 & 75.5 & 75.7 & 75.4 \\
    ProCo~\cite{du2024probabilistic} & 68.2 & 55.1 & 38.1 & 57.8 & 74.0 & 76.0 & 76.0 & 75.8 \\
    \midrule
    %Ours (Local Only) & 0.1 & 56.0 & 0.1 & 57.1 & 0.1 & 0.1 & 0.1 & 58.5 \\
    Baseline + Text & 70.6 & 58.0 & 42.1 & 60.7 & 74.8 & 76.4 & 76.3 & 76.2 \\
    Baseline + KD-I & 70.7 & 58.3 & 41.6 & 60.8 & 74.9 & 76.2 & 76.2 & 76.1 \\
    Baseline + RISE & 70.8 & 58.4 & 41.7 & 60.9 & 75.0 & 76.3 & 76.1 & 76.1 \\
    Baseline + KD-I-T & \textbf{71.0} & \textbf{60.1} & \textbf{43.2} & \textbf{62.0} & \textbf{75.4} & \textbf{76.7} & \textbf{76.5} & \textbf{76.5} \\
    \midrule
    Teacher model & 82.2 & 73.9 & 52.8 & 74.4 & 78.0 & 75.1 & 71.6 & 74.0 \\
    \bottomrule
  \end{tabular}
\end{table}

==> Tables/main_comb1.tex <==
\begin{table*}[t]
 \begin{minipage}{0.49\linewidth}
  \caption{Comparisons on Places-LT with ResNet-152. (* shows our reproduced result.)}
  \label{table:main_table_placelt}
  \centering
  \begin{tabular}{p{2.6cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}}
%   \begin{tabular}{llllll}
    \toprule
    Method & Many & Med & Few & Avg \\
    \midrule
    $\tau$ -norm~\cite{kang2019decoupling} & 37.8 & 40.7 & 31.8 & 37.9 \\
    Bal-Softmax & \textbf{42.0} & 39.3 & 30.5 & 38.6 \\
    ResLT~\cite{cui2022reslt} & 39.8 & 43.6 & 31.4 & 39.8 \\
    MiSLAS~\cite{zhong2021improving} & 39.6 & 43.3 & \textbf{36.1} & 40.4 \\
    PaCo~\cite{cui2021parametric} & 36.1 & \textbf{47.9} & 35.3 & 41.2 \\
    GPaCo~\cite{cui2023generalized} & 39.5 & 47.2 & 33.0 & \textbf{41.7} \\
    \midrule
    %Ours (Local Only) & 0.1 & 56.0 & 0.1 & 57.1 & 0.1 & 0.1 & 0.1 & 58.5 \\
    GPaco* & 36.1 & 48.0 & 36.5 & 41.5 \\
    GPaco* + Text & 36.7 & 48.6 & 37.7 & 42.2 \\
    GPaco* + KD-I & 37.0 & 48.5 & 37.3 & 42.2 \\
    GPaco* + RISE & 36.6 & 48.5 & 37.0 & 42.0 \\
    GPaco* + KD-I-T & \textbf{37.3} & \textbf{48.9} & \textbf{38.9} & \textbf{42.8} \\
    \midrule
    Teacher model & 51.6 & 48.5 & 36.2 & 47.2 \\
    \bottomrule
  \end{tabular}
\end{minipage}   
~
\begin{minipage}{0.49\linewidth}
  \centering
  \caption{Comparisons on ImageNet-LT with different
network architectures.}
  \label{table:main_table_diffarch}
  \begin{tabular}{p{2.6cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}}
%   \begin{tabular}{llllll}
    \toprule
    Method & Many & Med & Few & Avg \\
    \midrule
    Res-18 & 61.8 & 48.0 & 33.4 & 51.3 \\
    Res-18 + KD-I & 63.0 & 50.6 & 35.5 & 53.3 \\
    Res-18 + RISE & 63.1 & 50.8 & 35.8 & 53.5 \\
    Res-18 + KD-I-T & \textbf{64.2} & \textbf{51.5} & \textbf{38.3} & \textbf{54.6}\\
    \midrule
    Res-34 & 64.7 & 51.2 & 35.7 &  54.3 \\
    Res-34 + KD-I & 65.9 & 52.2 & 36.8 & 55.4 \\
    Res-34 + RISE & 65.7 & 52.3 & 37.3 & 55.5 \\
    Res-34 + KD-I-T & \textbf{67.5} & \textbf{54.3} & \textbf{41.0} & \textbf{57.6} \\
    \midrule
    LiVT (ViT-B/16) & 73.6 & 56.4 & 41.0 & 60.9 \\
    LiVT + KD-I & 77.0 & 60.7 & 38.8 & 64.0 \\
    LiVT + RISE & 76.9 & 60.9 & 39.1 & 64.1 \\
    LiVT + KD-I-T & \textbf{77.0} & \textbf{62.1} & \textbf{41.9} & \textbf{65.1} \\
    \bottomrule
  \end{tabular}
\end{minipage} 
\end{table*}

==> Tables/main_imglt_bak.tex <==
\begin{table*}[t]
 \begin{minipage}{\linewidth}
  \caption{Comparisons on ImageNet-LT with ResNet-50. (* shows our reproduced result.)}
  \label{table:main_table_imglt}
  \centering
  \begin{tabular}{p{6.5cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}}
%   \begin{tabular}{llllll}
    \toprule
    Method & Many & Med & Few & Avg \\
    \midrule
    $\tau$ -norm~\cite{kang2019decoupling} & 56.6 & 44.2 & 27.4 & 46.7  \\
    DisAlign~\cite{zhang2021distribution} & 61.3 & 52.2 & 31.4 & 52.9 \\
    GCL~\cite{li2022long} & 63.0 & 52.7 & 37.1 & 54.5 \\
    RIDE~\cite{wang2020long} & 66.2 & 51.7 & 34.9 & 54.9 \\
    BCL~\cite{zhu2022balanced} & - & - & - & 56.0  \\
    DOC~\cite{wang2022towards} & 65.1 & 52.8 & 34.2 & 55.0 \\
    DLSA~\cite{xu2022constructing} & 67.8 & 54.5 & 38.8 & 57.5 \\
    PaCo~\cite{cui2021parametric} & 64.4 & 55.7 & 33.7 & 56.0 \\
    NCL~\cite{li2022nested} & 67.3 & 55.4 & 39.0 & 57.7  \\
    GPaCo~\cite{cui2023generalized} & - & - & - & \textbf{58.5} \\
    ProCo~\cite{du2024probabilistic} & 68.2 & 55.1 & 38.1 & 57.8 \\
    \midrule
    %Ours (Local Only) & 0.1 & 56.0 & 0.1 & 57.1 & 0.1 & 0.1 & 0.1 & 58.5 \\
    %67.805, Med Prec@1: 55.052, Few Prec@1: 39.191
    ProCo* & 67.8 & 55.1 & 39.2 & 57.8 \\
    ProCo* + Text & 70.6 & 58.0 & 42.1 & 60.7 \\
    ProCo* + KD-I & 70.7 & 58.3 & 41.6 & 60.8\\
    ProCo* + RISE & 70.8 & 58.4 & 41.7 & 60.9\\
    ProCo* + KD-I-T & \textbf{71.0} & \textbf{60.1} & \textbf{43.2} & \textbf{62.0} \\
    \midrule
    Teacher model & 82.2 & 73.9 & 52.8 & 74.4 \\
    \bottomrule
  \end{tabular}
\end{minipage}   
~
\begin{minipage}{0.49\linewidth}
  \centering
  \caption{Comparisons on iNaturalist 2018 with ResNet-50. (* shows our reproduced result.)}
  \label{table:main_table_inat}
  \centering
  \begin{tabular}{p{2.55cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}}
%   \begin{tabular}{llllll}
    \toprule
    Method & Many & Med & Few & Avg \\
    \midrule
    $\tau$ -norm~\cite{kang2019decoupling} & 65.6 & 65.3 & 65.9 & 65.6  \\
    DisAlign~\cite{zhang2021distribution} & 69.0 & 71.1 & 70.2 & 70.6 \\
    GCL~\cite{li2022long} & 67.5 & 71.3 & 71.5 & 71.0 \\
    RIDE~\cite{wang2020long} & 72.2 & 70.2 & 72.2 & 72.7 \\
    BCL~\cite{zhu2022balanced} & 66.7 & 71.0 & 70.7 & 70.4 \\
    DOC~\cite{wang2022towards} & 72.8 & 71.7 & 70.0 & 71.0 \\
    DLSA~\cite{xu2022constructing} & - & - & - & 72.8 \\
    PaCo~\cite{cui2021parametric} & 70.3 & 73.2 & 73.6 & 73.2 \\
    NCL~\cite{li2022nested} & 72.0 & 74.9 & 73.8 & 74.2 \\
    GPaCo~\cite{cui2023generalized} & 73.0 & 75.5 & 75.7 & 75.4 \\
    ProCo~\cite{du2024probabilistic} & \textbf{74.0} & \textbf{76.0} & \textbf{76.0} & 
    \textbf{75.8} \\
    \midrule
    %Ours (Local Only) & 0.1 & 56.0 & 0.1 & 57.1 & 0.1 & 0.1 & 0.1 & 58.5 \\
    ProCo* & 70.8 & 73.2 & 72.6 & 72.7 \\
    ProCo* + Text  & 70.8 & 74.4 & 73.3 & 73.6 \\
    ProCo* + KD-I  & 70.9 & 74.5 & 73.2 & 73.6 \\
    ProCo* + RISE  & 70.8 & 74.3 & 73.0 & 73.4 \\
    ProCo* + KD-I-T & \textbf{71.0} & \textbf{74.5} & \textbf{74.2} & \textbf{74.0} \\
    \midrule
    Teacher model & 78.0 & 75.1 & 71.6 & 74.0 \\
    \bottomrule
  \end{tabular}
\end{minipage}
\end{table*}

==> Tables/main_scaling.tex <==
\begin{table*}[t]
  \centering
  \begin{tabular}{p{1.2cm}p{5.8cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}|p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}}
%   \begin{tabular}{llllll}
    \toprule
    & & \multicolumn{4}{c}{ResNet-50 (ProCo)} & \multicolumn{4}{c}{ViT-B/16 (LiVT)} \\
    \cmidrule(r){3-10}
    Method & Text Supervision & Many & Med & Few & Avg & Many & Med & Few & Avg \\
    \midrule
    KD-I-T & General Prompt & 71.0 & 60.1 & 43.2 & 62.0 & 77.0 & 62.1 & 41.9 & 65.1\\
    KD-I-T & General \& Targeted Prompt (Concat) & 70.9 & 60.0 & 43.1 & 61.9 & 76.9 & 61.9 & 40.8 & 64.8\\
    KD-I-T & General \& Targeted Prompt (Separate) & 71.0 & 60.2 & 45.1 & 62.3 & 77.1 & 62.7 & 41.1 & 65.3 \\
    KD-I-T & General \& Targeted Prompt (Shared) & \textbf{71.5} & \textbf{60.8} & \textbf{46.7} & \textbf{63.0} & \textbf{77.2} & \textbf{62.6} & \textbf{44.8} & \textbf{65.8} \\
    \bottomrule
  \end{tabular}
  \caption{Benefits of adding more text supervision.}
  \label{table:main_table_scale}
\end{table*}
